LiDAR-EDIT: LiDAR Data Generation by Editing the Object Layouts in Real-World Scenes

We present LiDAR-EDIT, a novel paradigm for generating synthetic LiDAR data for autonomous driving. Our framework edits real-world LiDAR scans by introducing new object layouts while preserving the realism of the background environment. Compared to end-to-end frameworks that generate LiDAR point clouds from scratch, LiDAR-EDIT offers users full control over the object layout, including the number, type, and pose of objects, while keeping most of the original real-world background. Our method also provides object labels for the generated data. Compared to novel view synthesis techniques, our framework allows for the creation of counterfactual scenarios with object layouts significantly different from the original real-world scene. LiDAR-EDIT uses spherical voxelization to enforce correct LiDAR projective geometry in the generated point clouds by construction. During object removal and insertion, generative models are employed to fill the unseen background and object parts that were occluded in the original real LiDAR scans. Experimental results demonstrate that our framework produces realistic LiDAR scans with practical value for downstream tasks.

==> control_strategy.tex <==
gm ,%\subsection{Runtime control strategy}
Our controller operates in a closed-loop fashion. We downsample the current, \(\curpcloud\), and goal point clouds, \(\goalpcloud\), to 1024 points using the furthest point sampling method from~\cite{Qi2017PointNet} before passing them through \DeformerNet{} to get the desired action. We use a resolved rate controller to compute the desired joint velocities following the desired end-effector displacement. %After the robot reaches an intermediate desired Cartesian position, it gets a new point cloud of the current object shape and repeats the process.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> intro_figure.tex <==
\setcounter{figure}{1}
\makeatletter
\let\@oldmaketitle\@maketitle% Store \@maketitle
\renewcommand{\@maketitle}{\@oldmaketitle % Update \@maketitle to insert...
  \begin{center}
    \centering
    \includegraphics[width=1.0\textwidth,height=3.25cm]{figures/figure_1_task.png}  
    \vspace{-18pt}
  \end{center}
  \footnotesize{\textbf{Fig.~\thefigure:\label{fig:sequence1}~Contextual Shape Servoing:} \ggn{} predicts a goal point cloud (green) by learning a model from human demonstrations. \DeformerNet{} uses the goal representation to compute actions to move the object to the desired shape, such that the human surgeon can cut the tissue at the desired location.}
  \vspace{-18pt}
  \medskip}
\makeatother
\maketitle
\thispagestyle{empty}
\pagestyle{empty}
